FRIED v2. A new grid of mass loss rates for externally irradiated protoplanetary discs

We present a new FRIED grid of mass loss rates for externally far-ultraviolet (FUV) irradiated protoplanetary discs. As a precursor to the new grid, we also explore the microphysics of external photoevaporation, determining the impact of polycyclic aromatic hydrocarbon (PAH) abundance, metallicity, coolant depletion (via freeze out and radial drift) and grain growth (depletion of small dust in the outer disc) on disc mass loss rates. We find that metallicity variations typically have a small effect on the mass loss rate, since the impact of changes in heating, cooling and optical depth to the disc approximately cancel out. The new FRIED grid therefore focuses on i) expanding the basic physical parameter space (disc mass, radius, UV field, stellar mass) ii) on enabling variation of the the PAH abundance and iii) including an option for grain growth to have occurred or not in the disc. What we suggest is the fiducial model is comparable to the original FRIED grid. When the PAH-to-dust ratio is lower, or the dust in the wind more abundant, the mass loss rate can be substantially lower. We demonstrate with a small set of illustrative disc evolutionary calculations that this in turn can have a significant impact on the disc mass/radius/ evolution and lifetime.

==> RefereeResponse.tex <==

We are grateful to the referee for their positive evaluation of the manuscript, and for insightful and probing comments that mean we now actually communicate why the results are the way they are, which was previously lacking. 

We believe that we have addressed all of the points raised. Changes to the manuscript are highlighted in bold and we summarise our changes below. 


\textbf{-	Abstract, last sentences
typos: can can → can
his → this}

\textit{Thank you, these typos have been corrected. 
}
\textbf{-	Introduction, 3rd paragraph
Readers would benefit from having defined threshold values for the high, intermediate, and low UV environments. This would provide clarity and assist them in better understanding the distinctions between these different UV conditions.}

\textit{For the first statement in that paragraph on statistical evidence we believe that it would be better to mention that it is the relative properties of discs that differ. E.g. rather than saying we see difference between low and high UV environments, saying we observe gradients. We have therefore changed the introduction 3rd paragraph to say that the properties of discs "vary as a function of the environmental UV field strength. }"

\textit{However, the terms high, intermediate and low UV fields are used throughout the paper so we agree these should be defined. Therefore, later in paragraph 3 of the introduction we add a footnote on this. Associated with this we also change our description of the van Terwisga and Hacar 2023 result as finding gradients in disc masses in "intermediate-to-low" UV environments. }

\textit{This comment also highlighted that the unit of FUV radiation field strength is not really defined in the submitted version of the paper, so we now highlight this in a footnote associated with paragraph 3.}

\textbf{-	Section 2
Does the torus-3DPDR code include H2 pumping? When the PAH-to-dust ratio is lowered, the heating could dominate over photoelectric heating with the interstellar radiation field spectrum.}

\textit{This is an interesting point. It also highlights that while we do not want to re-state all of the details of the calculations in this paper we should do a better job of highlighting where to find the relevant information. We now direct the reader to the original 3d-pdr paper (Bisbas et al. 2012), which describes the PDR microphysics details. }

\textit{In answer to this question, yes H2 pumping is included and the implementation is described in 2.6 of https://ui.adsabs.harvard.edu/abs/2012MNRAS.427.2100B/abstract. Looking at Figure 2 of Facchini + 2016 there appears to be other processes that would also provide higher heating than the H2 pumping. The effect on the mass loss rate by reduction in the PAH abundance is not going to be offset by additional heating from a secondary process, at least over the range of changes to PAH abundance considered here. }


\textbf{-	Eq.(3)
What is the underlying assumption on the stellar luminosity as a function of the stellar mass?}

\textit{This is simply based on an $L \propto M^4$ mass-luminosity relationship coupled with radiative equilibrium. It is admittedly simple, but changing this makes only a minor difference to the calculations. Arguably if treating the central sources in a more realistic fashion we would need to deal with pre main sequence evolutionary tracks which are time variable and hence adds a significant degree of additional complexity to the model that is unlikely to significantly affect mass loss rates. We have now mentioned where that assumed normalization scaling comes from in section 2. }



\textbf{-	Section 3.3, last paragraph
The authors employ the terms "small grains" and "grain growth" to characterize the two dust scenarios they adopted. However, this labeling might introduce ambiguity due to the lack of a precise definition for what "small" specifically entails in this context. I recommend using an alternative label, such as "ISM-like" or something similar, consistently throughout the paper. This would help avoid the ambiguity associated with the term "small grains" and provide clearer and more descriptive terminology for the two dust scenarios.}


\textit{Yes this is an excellent point. In discussion with potential users this terminology has already led to some confusion and this alternative labeling should help with that. We have followed the suggestion of adopting "ISM-like" and "grain growth"}



\textbf{-	Section 3.5.1, 1st paragraph
It is important to exercise caution and include a note about the possibility of EUV photoevaporation rates becoming dominant when the FUV photoevaporation rates are extremely low.}
\textbf{and} 
\textbf{-	Section 5.2, 4th paragraph
Is it possible for EUV photoevaporation rates to surpass FUV photoevaporation rates when the grid predicts values below 1e-10 Msun/yr?}


\textit{We respond to thse two points together since they both consider the possible role of the EUV. Firstly, Johnstone + 1998 do include an analytic estimate of the EUV driven mass loss rate. We have mentioned this at the end of 3.4, and also pointed to more recent work by Concha-Ramirez + that include that in disc evolutionary models. So if users wish to include that alongside FRIED they can. }

\textit{TJH: I am somewhat dubious about the reality of the EUV taking over again at large distances. Johnstone et al. 1998 were requiring super-critical flows, 1000\,K gas, and (quite reasonably) suggested a lower limit of 10$^4$\,G$_0$ as the lower limit that could lead to FUV driven flows. In the ONC that criterion implies the EUV dominates beyond around 0.3\,pc. Adams et al. (2004) demonstrated the sub-critical flows can be driven by much weaker FUV fields than $10^4$G$_0$ and, like us, see mass loss driven quite effectively by the FUV down to 2 orders of magnitude lower, and this is supported by other observations (e.g. van Terwisga \& Hacar 2023). Our model also goes beyond the 0.3pc in Figure 5 finding the EUV doesnt pick up in importance. The corresponding larger distances from the O star you would go to to get down below $\sim100\,$G$_0$ are beyond the extent of H\,\textsc{ii} region in the ONC. This does raise an interesting question of whether there can be very extended H\,\textsc{ii} regions with photoionised gas and low ($<100$\,G$_0$) FUV. Even then though, if you geometrically dilute the EUV at distances where the FUV is too weak to do anything and then calculate the column that can be ionised under ionisation equilibrium at typical outer disc densities you get an ionised layer of order only tens or hundreds of kilometres thick. E.g. in the ONC}
\begin{equation}
  \frac{N_{ly}}{4\pi D^2} \frac{1}{n^2\alpha_B} = \frac{10^{49}}{4\pi\times(0.3\textrm{pc})^2} \frac{1}{10^{18}\times 2.7\times10^{-13}} \sim 35\,km.
\end{equation}
\textit{and that ignores recombinations in any wind that would be driven
}
\textit{We have added a reduced version of this discussion to 3.4. 


\textbf{-	Section 3.4, 2nd paragraph
It would be beneficial to provide more specific information in this section about how the results are influenced by the PAH abundance and the chosen dust scenario. Additionally, a brief discussion on how the outcomes vary with these quantities would enhance the clarity and understanding of the findings.}


We have specified now that the FUV model in this initial exploration used $f_{PAH,d}=1$ and grain growth}. \textit{Ideally yes we would explore whether the same conclusion holds for all microphysics combinations we consider in the paper. However, given the objective here was to determine what to prioritise in a new grid rather than fully explore the possible combinations we would prefer to retain our small sample for now, which we think is also supported by the arguments made above. We have further added a statement saying that this was not an exhaustive study and looking into this further is something to be done in the future. }


\textbf{-	Section 3.1, last paragraph
What microphysics does the conclusion of “the more prudent parameter to vary is the PAH-to-dust mass ratio rather than metallicity” result from? More specifically, what are the major heating and cooling sources in the runs? I believe that dust-gas coupling serves as the primary coolant, which explains why the conclusion has been drawn; Both heating and cooling processes vary in proportion to the metallicity, whereas only heating is reduced when the PAH-to-dust ratio is lowered.}
\textbf{
and}

\textbf{-	Section 3.3, 2nd paragraph
What microphysics underlies the conclusion that there is no significant dependence on C depletion? Can readers interpret this result to mean that C I and C II are not major coolants?}

The referee makes a good point that our discussion of the details of the microphysics behind the behaviours seen in our explorative calculations are not thoroughly described. To help address this we have added a short paragraph just before 3.1 that summarises the main heating and cooling processes in the models. 

The referee is correct that CI and CII do play a secondary role. CO dominates the cooling for the inner flow and O dominates the cooling for the outer flow. Depleting oxygen could have a bigger impact on the mass loss rate (we chose carbon because it has been the focus of other work, e.g. Wölfer et al. 2019). The behavious described above are summarised in Figure 2 of Facchini et al. 2016 and we have confirmed this in our own models. Because depleting the oxygen abundance may have a more significant impact on the mass loss rate we have renamed the section "coolant depletion" to "carbon depletion" and commented on the possible importance of oxygen. 

The effect of varying metallicity is that you reduce the CO and O line cooling (and the other secondary coolants), and reduce the extinction in the wind, which all act to increase the mass loss rate. However that is almost balanced by the reduction in PAH heating. We have described this in 3.1 


\textbf{-	Eq.(6)
I believe that Eq.(5) should be multiplied on the right-hand side of Eq.(6), as that is the surface area heated by FUV in the torus-3DPDR simulations. If not, why is that justified?}

\textit{Yes this is correct, thank you for raising it. We have corrected this. 
}
\textbf{-	Description above Eq.(6)
Imposing half the energy-limited mass loss rates would lead to an overestimation, especially in weak FUV cases, as the deposited energy is largely distributed among kinetic energy and thermal energy (and, maybe, radiative cooling) rather than solely being used for mass loss. This point is worth being discussed more.}

\textit{Thank you for raising this. We have reduced this factor from 0.5 to 0.3, so using the upper end of efficiencies determined by Owen and Alvarez 2016. 
}
\textbf{-	Section 6.1, 2nd paragraph
The justification for the outer-disk-determining methods used by Concha-Ramirez et al. (2019) and Sellek et al. (2020) remains unclear. In reality, the outer disk should be located where Av (visual extinction) is approximately 1. The question arises whether these methods can consistently reproduce the Av ~ 1 location, irrespective of the PAH and dust parameters (PAH-to-dust ratio, metallicity, dust growth).}


\textit{The Sellek approach of using the location of maximum mass loss rate approximates to using the $\tau=1$ surface, since if the mass loss rate is lower at larger radii it is due to a low surface density. We have elaborated on this in 6.1.}
